A Reinforcement Learning Approach to Synthetic Data Generation

Synthetic data generation (SDG) is a promising approach for enabling data sharing in biomedical studies while preserving patient privacy. Yet, state-of-the-art generative models often require large datasets and complex training procedures, limiting their applicability in small-sample settings common in biomedical research. This study aims to develop a more principled and efficient approach to SDG and evaluate its efficacy for biomedical applications. In this work, we reframe SDG as a reinforcement learning (RL) problem and introduce RLSyn, a novel framework that models the data generator as a stochastic policy over patient records and optimizes it using Proximal Policy Optimization with discriminator-derived rewards. We evaluate RLSyn on two biomedical datasets--AI-READI and MIMIC-IV--and benchmark it against state-of-the-art generative adversarial networks (GANs) and diffusion-based methods across extensive privacy, utility, and fidelity evaluations. On MIMIC-IV, RLSyn achieves predictive utility comparable to diffusion models (S2R AUC 0.902 vs 0.906 respectively) while slightly outperforming them in fidelity (NMI 0.001 vs. 0.003; DWD 2.073 vs. 2.797) and achieving comparable, low privacy risk (~0.50 membership inference risk AUC). On the smaller AI-READI dataset, RLSyn again matches diffusion-based utility (S2R AUC 0.873 vs. 0.871), while achieving higher fidelity (NMI 0.001 vs. 0.002; DWD 13.352 vs. 16.441) and significantly lower vulnerability to membership inference attacks (AUC 0.544 vs. 0.601). Both RLSyn and diffusion-based models substantially outperform GANs across utility and fidelity on both datasets. Our results suggest that reinforcement learning provides a principled and effective approach for synthetic biomedical data generation, particularly in data-scarce regimes.

==> tables/utility_results.tex <==
\begin{table}[h!]
    \centering
    \caption{Utility results measured via classification performance of models trained on the synthetic data and tested on the real data. Performance was measured using Area under the receiver operating characteristic curve (AUC). The best performance for each metric is bolded.}
    \begin{tabular}{c|cc|cc}
        \toprule
        \multicolumn{1}{c|}{} & 
        \multicolumn{2}{c|}{\textbf{MIMIC-IV}} & 
        \multicolumn{2}{c}{\textbf{AI-READI}} \\
        \cmidrule{1-5}
        
          & \textbf{S2R} & \textbf{R2S} & \textbf{S2R} & \textbf{R2S} \\
        \cmidrule{1-5}
        EMR-WGAN & 0.764 $\pm$ 0.025 & 0.666 $\pm$ 0.063 & 0.747 $\pm$ 0.031 & 0.619 $\pm$ 0.046\\
        EHRDiff & 0.906 $\pm$ 0.001 & 0.896 $\pm$ 0.002 & 0.871 $\pm$ 0.011 & 0.901 $\pm$ 0.004\\
        \modelname & 0.902 $\pm$ 0.001 &0.909 $\pm$ 0.005 & 0.873 $\pm$ 0.021 & 0.868 $\pm$ 0.011\\
        \cmidrule{1-5}
        \multicolumn{1}{c|}{Real Baseline} & 
        \multicolumn{2}{c|}{0.919 $\pm$ 0.001} & 
        \multicolumn{2}{c}{0.870 $\pm$ 0.004} \\
        
        \bottomrule
    \end{tabular}
    \label{tab:grouped}
\end{table}

